A Comprehensive Study on Deep Learning Bug Characteristics

Deep learning has gained substantial popularity in recent years. Developers mainly rely on libraries and tools to add deep learning capabilities to their software. What kinds of bugs are frequently found in such software? What are the root causes of such bugs? What impacts do such bugs have? Which stages of deep learning pipeline are more bug prone? Are there any antipatterns? Understanding such characteristics of bugs in deep learning software has the potential to foster the development of better deep learning platforms, debugging mechanisms, development practices, and encourage the development of analysis and verification frameworks. Therefore, we study 2716 high-quality posts from Stack Overflow and 500 bug fix commits from Github about five popular deep learning libraries Caffe, Keras, Tensorflow, Theano, and Torch to understand the types of bugs, root causes of bugs, impacts of bugs, bug-prone stage of deep learning pipeline as well as whether there are some common antipatterns found in this buggy software. The key findings of our study include: data bug and logic bug are the most severe bug types in deep learning software appearing more than 48% of the times, major root causes of these bugs are Incorrect Model Parameter (IPS) and Structural Inefficiency (SI) showing up more than 43% of the times. We have also found that the bugs in the usage of deep learning libraries have some common antipatterns that lead to a strong correlation of bug types among the libraries.

==> Feature.tex <==
\subsubsection{Feature Bug}
%Specification problems usually create corresponding feature problems. A feature can be wrong, missing, or superfluous. A missing feature or case is the easiest to detect and correct. A wrong feature could have deep design implications. Extra features were once considered desirable. We now recognize that “free” features are rarely free. Any increase in generality that does not contribute to reliability, modularity, maintainability, and robustness should be suspected. Gratuitous enhancements can, if they increase complexity, accumulate into a fertile compost heap that breeds future bugs, and they can create holes that can be converted into security breaches. Conversely, one cannot rigidly forbid additional features that might be a consequence of good design. Removing the features might complicate the software, consume more resources, and foster more bugs. 

==> Memory.tex <==
\subsubsection{Memory Bug}
Often ML models are built in a way such that the program halts upon excessive use of the programming memory. In such cases, the user will not be aware of this incident until runtime, since this issue will not be exhibited during the compilation phase. Memory bugs are not easy to find or debug as they only reveal themselves duing runtime. Since an infected code will take considerable time to execute, a huge amount of effort will thus be invested in their detection and resolution. 
For example, in the following code snippet
\footnote{\url{https://stackoverflow.com/questions/31467487}}, the code encounters a memory error during a large size of the training dataset.
\begin{lstlisting}[language = python]
import numpy as np
from sklearn.cross_validation import train_test_split

X = np.random.random((10000,70000))
Y = np.random.random((10000,))
X_train, X_test, Y_train, Y_test = train_test_split(X, Y, test_size = 0.33, random_state=42)
\end{lstlisting}
To solve this problem, the training dataset has to be split and fed into the ML model or the data needs to be shuffled prior to further processing.

==> Requirement.tex <==
\subsubsection{Requirement and Specification Bug}
%Requirements and the specifications developed from them can be incomplete, ambiguous, or self-contradictory. They can be misunderstood or impossible to understand. The specification may assume, but not mention, other specifications and prerequisites that are known to the specifier but not to the designer. And specifications that don’t have these flaws may change while the design is in progress. Features are modified, added, and deleted. The designer has to hit a moving target and occasionally misses. Requirements, especially as expressed in a specification (or often, as not expressed because there is no specification) are a major source of expensive bugs. The range is from a few percent to more than 50%, depending on application and environment. What hurts most about these bugs is that they’re the earliest to invade the system and the last to leave. It’s not unusual for a faulty requirement to get through all development testing, beta testing, and initial field use, only to be caught after hundreds of sites have been installed.
%-To Do if we find any bug of this category.

==> Requirement_.tex <==
abcd

==> Requirement_and_Specifications.tex <==
abcd

==> Structural_Bug.tex <==
\subsubsection{Structural Bug}
Abcd


==> Structure.tex <==
\subsubsection{Structure Bug}
A vast majority of the ML bugs are generated due to incorrect definitions of the ML model's structure. These include mismatch of dimensions between different layers of ML models, the presence of anomaly between the training and test datasets, use of incorrect data structures in implementing a particular function, etc. Structural bugs also consist of erroneous ordering of different layers during the built of an ML model. Construction of the structure broadly depends on the calculated size of the input and corresponding output of each layer. For example, in the following code snippet
\footnote{\url{https://stackoverflow.com/questions/42621652}}, the shape of the layers are inconsistent with each other.
\begin{lstlisting}[language = python]
.....
Shape must be rank 2 but is rank 3 for 'MatMul_3' (op: 'MatMul') with input shapes: [100,?,400], [400,2].
\end{lstlisting}
These problems are typically generated when the user is unaware of the model's structure and the process of defining the size of the different layers.

==> TODO.tex <==
\section{TODO}
\begin{enumerate}
	\item \st{Section 4  Deadline }(12 January) \wa{Rangeet}
	\item \st{Section 5 Deadline (12 January)} \wa{Johir} 
	\item \st{Related Works and Introduction } \wa{Probably Giang}
	\item \st{Threat to Validity deadline 13 January} \wa{Johir}
	\item Discussion Section Deadline (January 15) \wa{Johir} 
	\item Section 7  Deadline (15 January) \wa        {Johir}
	\item \st{Section 2 Johir and Giang }
	\item Think about coherency (All and discuss regularly)
\end{enumerate}

==> blackboxabstraction.tex <==
\subsection{Blackbox abstraction can be potemkin village}
\findings{88/377 bugs occur due to the effect of black box abstraction in ML APIs}{arg2}
In this section we describe the drawbacks of backbox abstraction and ML programming. Our study shows that blackbox abstraction tends to increase technical difficulty among ML programmers. 
Though abstraction is an important concept for high producity among software engineers, ML programming tends to show a negative effect due to to the adaption of existing concepts of abstraction directly. 
In our study, we have seen \textbf{88/377} bugs are due to the blackbox abstraction. Blackbox astraction hides the details of the ML process to the programmer and the programmer does not have any useful information from the front side of the wall to debug the program.

% https://stackoverflow.com/questions/47594861/predicting-a-multiple-forward-time-step-of-a-time-series-using-lstm

% https://stackoverflow.com/questions/44852153/layer-called-with-an-input-that-isnt-a-symbolic-tensor-keras
For example, in the following code snippet \footnote{\url{https://stackoverflow.com/questions/47932589}} the poster is trying to train an RNN model for estimating the sine wave frequency. 
\begin{lstlisting}[language = python]
from keras.models import Model
from keras.layers import Dense, Input, LSTM

input_series = Input(shape=(2000,),name='Input')
dense_1 = Dense(100)(input_series)
pred = Dense(1, activation='relu')(dense_1)
model = Model(input_series, pred)
model.compile('adam','mean_absolute_error')
model.fit(train_x[:100], train_y[:100], epochs=100)
\end{lstlisting}
The model looks perfectly fine from the front but actually is not learning anything in the process. The develoepr doesn't have any information how the data is flowing, how different layers are behaving, what is the effect of changing the data on the learning process, changing the frequency of data in the learning process e.t.c. 

Opinion from expert suggests some data cleaning, changning the loss function, adding some droput layers which can not be understood from the front end without looking at the behavior of the process at different epochs and also looking at the data flow through the graph.

Programmers also face difficulty to understand the data shapes and types being converted by one abstract API and connecting the output that API to the next layers. The abstraction hides these details information from the programmers creating difficulties to debug. 
For example, in the following code snippet \footnote{\url{https://stackoverflow.com/questions/36428323}} putting the output from Line 3 to Line 4 causes the program to crash. 
\begin{lstlisting}[language = python]
sequence = Input(shape=(max_sent_len,), dtype='int32')
embedded = Embedding(vocab_size, word_embedding_size)(sequence)
lstm = LSTM(hidden_state_size, activation='sigmoid', inner_activation='hard_sigmoid', return_sequences=True)(embedded) 
pool = AveragePooling1D()(lstm)
output = Dense(1, activation='sigmoid')(pool)
\end{lstlisting}
To fix the problem the user had to add the following line:
\begin{lstlisting}[language = python]
distributed = TimeDistributed(Dense(1))(lstm)
\end{lstlisting}

after Line 3 and pass that output to \code{AveragePooling1D()} at Line 5.
\begin{lstlisting}[language = python]
sequence = Input(shape=(max_sent_len,), dtype='int32')
embedded = Embedding(vocab_size, word_embedding_size)(sequence)
lstm = LSTM(hidden_state_size, activation='sigmoid', inner_activation='hard_sigmoid', return_sequences=True)(embedded)
distributed = TimeDistributed(Dense(1))(lstm)
pool = AveragePooling1D()(distributed)
output = Dense(1, activation='sigmoid')(pool)
\end{lstlisting}

The user does not have information from the code what kind of conversion is being done to the data at the backend. The behavior may be even different for different kinds of data. 


==> dimension.tex <==
\subsection{Dimension mismatch may appear due to different operations in DNN}
\findings{44/377 bugs are related to dimension mismatch in DNN}{arg2}
Dimension mismatch related problems may appear due to the mismatch of data shape with input layer dimension of the network or due to the change of dimension due to different operations in the DNN.
For example, if the dimension of the input layer is $n$ and the number of features in the data are $m  != n$ then the program will show dimension mismatch error. For example, in the following code snippet \footnote{\url{https://stackoverflow.com/questions/39376169/}} in the program was failing at the input layer with dimension mismatch
\begin{lstlisting}
....
img_width, img_height = 150, 150
model = Sequential()
model.add(Convolution2D(32, 3, 3, input_shape=(3, img_width, img_height)))
...
\end{lstlisting}
because the \code{input_shape = (3,150,150)} but the test images sizes were \code{150*198} pixel.
DNN operations like \code{flattening, convolution, polling, reshaping} can change the dimensions creating possibility of dimension mismatch if the programmer is not careful.

==> hyperparam.tex <==
\subsection{Absence of suggestions in chosing hyper parameters}
\findings{58/377 posts can be related to the need for suggestions to chose hyper parameters}{arg2}
%https://stackoverflow.com/questions/39217567/
ML programmers often need to chose the most optimal hyper parameters to get better performance. These parameters can be varied for different problem type. For one problem scenario, the user might needs to use 
\code{binary_crossentropy} to get better performance and in other other kind of problem the loss function may be \code{crossentropy}, \code{mse} etc.
Even for the choice of activation functions, the user needs to be careful. For some layer \code{relu} may be the best activation function for for other layers it may not be. Dpending on the type of problem either classification or regression the parameters may need to be varied. Also depending on the properties of the data the parameters need wise choice. But current ML APIs give no hints on these kinds of choice. The user could successfully train the model but gets very poor performance without getting any error or warning. For example, in the following code snippet \footnote{\url{https://stackoverflow.com/questions/39217567/}}
\begin{lstlisting}[language = python]
....
# Compile model
model.compile(loss='mse', optimizer='SGD', metrics=['accuracy'])
# Fit the model
model.fit(X, y, nb_epoch=1000, batch_size=50, verbose=0)
# evaluate the model
scores = model.evaluate(X, y)
print("%s: %.2f%%" % (model.metrics_names[1], scores[1]*100))
output = model.predict(X)
\end{lstlisting}
the poster gets less than 60\% of prediction accuracy which was surprizing. Based on expert suggestions, the change of the loss to \code{binary_crossentropy} at Line 3, decreasing the deafult learning rate of the optimizer , decreasing the epoch and adding dropout layers to the model.


==> misusedata.tex <==
\begin{figure*}[t]
	\includegraphics[width= \linewidth]{problemstages.png}
	\caption{API Misuses accross different ML Stages \cite{stages}}
	\label{fig:misusechart}
\end{figure*}

==> pcomb.tex <==
\subsection{Combination of parameters can lead to suboptimal performance}

Sometime a combination of hyper parameter might be the culprit for creating bad performance. We have found six posts on our dataset talking about bad combination of hyper parameters. 
For example, in the following code snippet
\begin{lstlisting}[language = python]
...
model.add(Dense(output_dim = 1, activation = "softmax"))
model.compile(optimizer = "adam", loss = "categorical_crossentropy")
model.fit(X_train, y_train, batch_size = batch_size, nb_epoch = nb_epochs, show_accuracy = True, verbose = 2, validation_data = (X_test, y_test))
score = model.evaluate(X_test, y_test, show_accuracy = True, verbose = 0)
...
\end{lstlisting}
using \code{softmax} activation function at the output layer when \code{output_dim = 1} causes to model to perform very badly. Also the \code{categorical_crossentropy} is not the optimal choice for tis problem rather \code{binary_crossentropy} has the evidence to perform better from the expert opinions. 




==> redundant.tex <==
\subsubsection{Classification of the bugs}
To classify the bug types we followed the classification from some already
existing literature and appended on top of that. The added types were based on
the data that we studied and followed an open coding scheme. The third author studied the posts initially to come up with the possible bug types. We
followed the pilot study to check whether the manual labelling is working properly under the supervision of the first author and followed open coding scheme to check whether the classification criteria is standard or not for deep learning bugs. 

\subsubsection{Classification of the bugs into deep learning stages}
Deep learning process can be divided into seven stage pipeline \cite{stages}.
The stages are data collection, data preparation, choice of model, training,
evaluation, hyper parameter tuning, prediction. Among the seven stages, the first
one is not related to programming. The other stages are related to programming
and are supported by the deep learning libraries through their APIs. 
We use these stages to classify the bugs into different stages. 
\subsubsection{Classification of the effect of bugs}
The bugs may have different effects. A suervised pilot study and open coding schemes were
used to identify the effects that are possible through these bugs. 

==> tightcoupling.tex <==
\subsection{Tight coupling between data and model}
\findings{ML has tight coupling between data and model}{arg2}
In machine learning a model may be performing well for a particular kind of data but fails for a different dataset. 
In our study we found \textbf{8} different posts talking about trying to reuse a model or some components from a good model to the new dataset and all of them leading to very bad perfromance or error. 
This weakness is is exploited for adversarial attacks in machine learning as well. Small change in the dataset can cause the total failure of the model. Chaning of data can lead to degradation of performance as well as run time failure. For example, in the following code snippet \footnote{\url{https://stackoverflow.com/questions/43900125/}} the user tries to resuse an image classification model (for classification of two images) to a dataset of 4 different images.
\begin{lstlisting}[language = python]
....
conv11 = Conv2D(4, (1, 1), activation='softmax')(conv10)
model = Model(inputs=[inputs], outputs=[conv11])
\end{lstlisting}
The user tries to change the dimension of the output layer to 4 ultimately leading to bad performance. 


==> trainmonitor.tex <==
\subsection{Absence of the training process monitoring}
\findings{80/377 posts talk about bugs that appear due to the absence of well developed monitoring tools at the runtime}{arg2}
The current monitoring tools only output some logs showing some accuracies and loss values at the runtime, some good monitors also show visualizations. But the programmer does not know why  these values are appearing and which block or node in the network or model is causing this problem. 
For example, in the follwoing code snippet \footnote{\url{https://stackoverflow.com/questions/33969059}} 
\begin{lstlisting}
Epoch 1/20
100000/100000 [==============================] - 0s - loss: 60726734.3061 - acc: 1.0000     
..... 
Epoch 20/20
100000/100000 [==============================] - 0s - loss: 60726734.3061 - acc: 1.0000     

\end{lstlisting}
the training output shows a huge amount of loss at the very first epoch and also shwoing 100\% accuracy which is contradictory and wrong. 
We notice the scenario is same even at the 20th epoch having the same value of loss and accuracy. 
The user is not getting any error but the whole process of training the model with the dataset is going wrong. The user does not know why this is happening and what piece in the training process is malfunctioning. 

==> typecheck.tex <==
\subsection{Absence of type checking}
\findings{65/377 bugs are caused due to type mismatch}{arg2}
In machine learning type checking problems appear very often. 
Our study reveals that almost  \textbf{17\%} bugs are due to type mistmatch. The user even can not solve these problems by working on the code which leads them to ask on \sof. Our filtering to only study the posts that are of score greater than 5 ensures that these posts are not mere silly novice problems. 
For example, a programmer is trying a train a model \footnote{\url{https://stackoverflow.com/questions/35968973/}} where the data are in \code{DataFrame} format using \code{Keras} library. 
\begin{lstlisting}[language = python]
model.fit(trainx, trainy, nb_epoch=20, batch_size=16)
Epoch 1/20
Traceback (most recent call last):
.........
IndexError: indices are out-of-bounds
\end{lstlisting}
The problem is solved by converting the \code{DataFrame} to \code{numpy} array. Due to this type problem the whole program crashes at the first epoch of the training process but the user does not have any clue why this is happening. Even the runtime error message \code{IndexError: indices are out-of-bounds} is misleading here.

Sometimes more than one library are used together. For example, \keras and \tensor are often used simulataneously in ML programs. The programmers are also often bombarded with the type mismatch appearing due to this combination. For example, the following code snippet 
\begin{lstlisting}[language = python]
left = Activation('relu')(img)
right = Activation('relu')(tf.mul(img, -1.0))
\end{lstlisting}
raises the following exception at the runtime:
\begin{lstlisting}[language = python]
TypeError: Output tensors to a Model must be Keras tensors. Found: Tensor("add_1:0", shape=(?, 5, 1, 3), dtype=float32)
\end{lstlisting}
This happens because a \tensor \code{Tensor} is passed to a \keras API, which is rather programmed to operate with \keras \code{Tensor}. These kind of errors appear both due to the effect of blackbox abstraction as well as the absence of proper type checking. 

==> versioning.tex <==
\subsection{Absence of backward compatibility while versioning}

In ML libraries APIs upgrade are often seen to break the codes from previous version. In our study we have found 14 posts talking about bugs in the program created due to the upgrade of library. 
For example, in the following code snippet \footnote{\url{https://stackoverflow.com/questions/42441431/}}
\begin{lstlisting}[language = python]
tf_embedding_input = ...    # pre-processing output tensor
# Keras model
model = Sequential()
e = Embedding(max_features, 128, input_length=maxlen)
### THIS DOESN'T WORK ANYMORE ###
e.set_input(tf_embedding_input)
\end{lstlisting}
the user asks about the error created in the code after upgrading to new version. The API that used to work in the last version is completely removed causing the program to fail. This kind of scenario may be more problematic in large code base. The whole legacy code may stop working after upgrading the system to new version. 
